Towards Better Understanding of Contrastive Sentence Representation Learning: A Unified Paradigm for Gradient

Sentence Representation Learning (SRL) is a crucial task in Natural Language Processing (NLP), where contrastive Self-Supervised Learning (SSL) is currently a mainstream approach. However, the reasons behind its remarkable effectiveness remain unclear. Specifically, many studies have investigated the similarities between contrastive and non-contrastive SSL from a theoretical perspective. Such similarities can be verified in classification tasks, where the two approaches achieve comparable performance. But in ranking tasks (i.e., Semantic Textual Similarity (STS) in SRL), contrastive SSL significantly outperforms non-contrastive SSL. Therefore, two questions arise: First, *what commonalities enable various contrastive losses to achieve superior performance in STS?* Second, *how can we make non-contrastive SSL also effective in STS?* To address these questions, we start from the perspective of gradients and discover that four effective contrastive losses can be integrated into a unified paradigm, which depends on three components: the **Gradient Dissipation**, the **Weight**, and the **Ratio**. Then, we conduct an in-depth analysis of the roles these components play in optimization and experimentally demonstrate their significance for model performance. Finally, by adjusting these components, we enable non-contrastive SSL to achieve outstanding performance in STS.

==> application <==
\section{Application to Ineffective Objectives}
\label{sec:application}

After understanding the properties that the gradients of the effective losses in SRL should possess, we can make some ineffective optimization objectives effective by adjusting their gradients. 

Alignment and uniformity~\citep{wang_understanding_2020} are two metrics used to assess the performance of the representation space, yet directly using them as optimization objectives results in poor performance. Alignment can be represented as
\begin{align*}
    \mathcal{L}^\mathrm{a} = \frac{1}{N}\sum_{i=1}^N\|h_i-h_i'\|_2^2,
\end{align*}
and uniformity can be represented in many forms~\citep{liu_learning_2021}, one of which is the Minimum Hyperspherical Energy (MHE)
\begin{align*}
    \mathcal{L}^\mathrm{u,MHE}=\log\frac{2}{N(N-1)}\sum_{1\le k< l\le N}e^{-\|h_k-h_l\|_2^2},
\end{align*}
and another is the Maximum Hyperspherical Separation (MHS)
\begin{align*}
    \mathcal{L}^\mathrm{u,MHS}_i=-\min_{j\neq i}\|h_i-h_j\|_2.
\end{align*}

Non-contrastive self-supervised learning is popular in visual representation learning, yet its performance is relatively poor when applied to sentence representation learning. Common optimization objectives in this direction include Barlow Twins
\begin{align*}
    \mathcal{L}^\mathrm{B}=\sum_{k=1}^D(W_{kk}-1)^2+\lambda\sum_{k\neq l}^DW_{kl}^2,
\end{align*}
where $W=\frac{1}{N}\sum_{i=1}^Nh_ih_i'^\top$, and VICReg
\begin{align*}
    \mathcal{L}^\mathrm{V}=\mathcal{L}^\mathrm{V}_1+\mathcal{L}^\mathrm{V}_2+\mathcal{L}^\mathrm{V}_2,
\end{align*}
where
\begin{gather*}
    \mathcal{L}^\mathrm{V}_1=\frac{1}{N}\sum_{i=1}^N\|h_i-h_i'\|_2^2,\ 
    \mathcal{L}^\mathrm{V}_2=\frac{\lambda_1}{D}\sum_{k\neq l}^DW_{kl}^{'2},\\
    W'=\frac{1}{N-1}\sum_{i=1}^N(h_i-\bar{h}_i)(h_i'-\bar{h}_i')^\top,\\
    \mathcal{L}^\mathrm{V}_3=\frac{\lambda_2}{D}\sum_{k=1}^D\max(0,\gamma - \mathrm{std}(h_i)_k).
\end{gather*}

The gradient w.r.t $h_i$ for alignment and uniformity ($\mathcal{L}^\mathrm{a\&u}=\mathcal{L}^\mathrm{a} + \lambda \mathcal{L}^\mathrm{u}$) and non-contrastive self-supervised learning ($\mathcal{L}^\mathrm{B}$ and $\mathcal{L}^\mathrm{V}$) can also be mapped into the paradigm. We present the results in Table~\ref{tab:ineffective_objectives}, where the gradient for non-contrastive self-supervised learning is the equivalent form derived by \citet{tao_exploring_2022}. Furthermore, we have omitted the gradient dissipation term in the table, as this term is constant at 1 across all gradients. 

\begin{table}[ht]\small
  \centering
    \begin{tabular}{c|l|l}
    \toprule
    \textbf{Type}  & \multicolumn{1}{c|}{\textbf{Weight}} & \multicolumn{1}{c}{\textbf{Ratio}} \\
    \midrule
    MHE   
    & 
    $
    \begin{aligned}
        \frac{2\lambda e^{2h_i^\top h_j}}{\sum_{1\le k < l\le N}e^{2h_k^\top h_l}}
    \end{aligned}
    $
    &  
    $
    \begin{aligned}
        \frac{\sum_{1\le k< l\le N}e^{2h_k^\top h_l}}{\lambda N\sum_{k\neq i}^Ne^{2h_i^\top h_k}}
    \end{aligned}
    $
    \\
    MHS   
    &  
    $
    {\scriptsize\left\{\begin{aligned}
        &\lambda/\|h_i-h_j\|_2,\quad\mathrm{else}\\
        &0,j\neq\arg\max_{k\neq i}h_i^\top h_k
    \end{aligned}\right.}
    $
    &  
    $
    \begin{aligned}
        \frac{2\|h_i-h_j\|_2}{\lambda N}
    \end{aligned}
    $
    \\
    BT 
    & 
    $
    \begin{aligned}
        2\lambda h_i'^\top h_j'/N^2
    \end{aligned}
    $
    &  
    $
    % \begin{aligned}
        \frac{N(I-(1-\lambda)W_\mathrm{diag})}{\lambda\sum_{k\neq i}^N h_i'^\top h_k'}
    % \end{aligned}
    $
    \\
    VICReg    
    &       
    $
    \begin{aligned}
        2\lambda h_i^\top h_j/N^2
    \end{aligned}
    $
    &  
    $
    % \begin{aligned}
    % \frac{N}{\lambda\sum_{k\neq i}^N h_i^\top h_k}
    % \end{aligned}
    N / (\lambda\sum_{k\neq i}^N h_i^\top h_k)
    $
    \\
    \bottomrule
    \end{tabular}%
  \caption{[TODO]$W_\mathrm{diag}$ is the diagonal matrix of $W$.}
  \label{tab:ineffective_objectives}%
\end{table}%

Components in the paradigm of ineffective losses do not perform in the same manner as those of effective losses. For the gradient dissipation term, since its value is 1 in all ineffective losses, it implies that it has no effect. For the weight term, except for MHS, other losses cannot ensure that the hardest negative samples dominate in the gradient. For the ratio term, these losses fail to guarantee an appropriate value, and Barlow Twins even distorts the optimization direction from the positive sample. Therefore, we attempt to make these losses effective by adjusting these terms. Note that when modifying Barlow Twins and VICReg, the equivalent forms provided by ~\citet{tao_exploring_2022} are utilized:
\begin{align*}
    \mathcal{L}^\mathrm{eB}_i=-h_i^\top w_{\mathrm{p},i}^\mathrm{B}h_i'+\lambda\sum_{j\neq i}^Nh_i^\top w_{\mathrm{n},ij}^\mathrm{B}h_j,
\end{align*}
where $w_{\mathrm{p},i}^\mathrm{B}=\frac{2(I-(1-\lambda)W_\mathrm{diag})}{N}, w_{\mathrm{n},ij}^\mathrm{B}=\frac{2h_i'^\top h_j'I}{N^2}$;
\begin{align*}
    \mathcal{L}^\mathrm{eV}_i=-h_i^\top w_{\mathrm{p},i}^\mathrm{V}h_i'+\lambda\sum_{j\neq i}^Nh_i^\top w_{\mathrm{n},ij}^\mathrm{V}h_j,
\end{align*}
where $w_{\mathrm{p},i}^\mathrm{V}=\frac{2I}{N}, w_{\mathrm{n},ij}^\mathrm{V}=\frac{2h_i^\top h_jI}{N^2}$, and all $w_{\mathrm{p},i}^\mathrm{B}, w_{\mathrm{n},ij}^\mathrm{B}, w_{\mathrm{p},i}^\mathrm{V}, w_{\mathrm{n},ij}^\mathrm{V}$ do not require gradient.

To adjust the gradient dissipation term, we stop the gradient of anchor $h_i$ that do not meet the condition ($h_i^\top h_i' - \max_{k\neq i}^N h_i^\top h_k' < m$), which is equivalent to multiplying the loss by the indicator function
\begin{align*}
    d_i = \mathbb{I}_{\{h_i^\top h_i'-\max_{k\neq i}^Nh_i^\top h_k'<m\}}.
\end{align*}
To adjust the weight term, we first set $\lambda=1$. Then, we introduce a temperature parameter $\tau$ to $\mathcal{L}^\mathrm{u,MHE}$:
\begin{align*}
    \mathcal{L}^\mathrm{u,mMHE}=\log\frac{2\sum_{1\le k< l\le N}e^{-\|h_k-h_l\|_2^2/\tau}}{N(N-1)},
\end{align*}
and modify $w_{\mathrm{n},ij}^\mathrm{B}$ and $w_{\mathrm{n},ij}^\mathrm{V}$ to an exponential form:
\begin{align*}
    w_{\mathrm{n},ij}^\mathrm{mB}=\frac{e^{h_i'^\top h_j'/\tau}}{\sum_{k\neq l}e^{h_k'^\top h_l'/\tau}},
    w_{\mathrm{n},ij}^\mathrm{mV}=\frac{e^{h_i^\top h_j/\tau}}{\sum_{k\neq l}e^{h_k^\top h_l/\tau}}.
\end{align*}
To adjust the ratio term, we modify all losses to have a static ratio $r$. For alignment and uniformity, we prepend a coefficient
to the alignment:
\begin{gather*}
   \mathcal{L}_i^\mathrm{a,mMHE}=\underbrace{\frac{r\sum_{j\neq i}^Ne^{2h_i^\top h_j/\tau}}{\tau \sum_{1\le k<l\le N}e^{2h_k^\top h_l/\tau}}}_\mathrm{no\ gradient}
   \|h_i-h_i'\|_2^2,\\
   \mathcal{L}_i^\mathrm{a,mMHS}=\underbrace{\frac{r}{2\max_{j\neq i}^N\|h_i-h_j\|_2}}_\mathrm{no\ gradient}\|h_i-h_i'\|_2^2.
\end{gather*}
For non-contrastive self-supervised learning, we modify $w_{\mathrm{p},i}^\mathrm{B}$ and $w_{\mathrm{p},i}^\mathrm{V}$ to
\begin{align*}
    w_{\mathrm{p},i}^\mathrm{mB}=\frac{r\sum\limits_{j\neq i}^Ne^{h_i'^\top h_j'/\tau}}{\sum_{k\neq l}e^{h_k'^\top h_l'/\tau}},
    w_{\mathrm{p},i}^\mathrm{mV}=\frac{r\sum\limits_{j\neq i}^Ne^{h_i^\top h_j/\tau}}{\sum_{k\neq l}e^{h_k^\top h_l/\tau}}, 
\end{align*}
both of which do not require gradients as well. Finally, the modified losses can be represented as
\begin{gather}
    \mathcal{L}_i^\mathrm{mMHE}=d_i(\mathcal{L}_i^\mathrm{a,mMHE}+\mathcal{L}^\mathrm{u,mMHE}),\\
    \mathcal{L}_i^\mathrm{mMHS}=d_i(\mathcal{L}_i^\mathrm{a,mMHS}+\mathcal{L}_i^\mathrm{u,MHS}),\\
    \mathcal{L}_i^\mathrm{mB}=d_i(-h_i^\top w_{\mathrm{p},i}^\mathrm{mB}h_i'+\lambda\sum_{j\neq i}^Nh_i^\top w_{\mathrm{n},ij}^\mathrm{mB}h_j),\\
    \mathcal{L}_i^\mathrm{mV}=d_i(-h_i^\top w_{\mathrm{p},i}^\mathrm{mV}h_i'+\lambda\sum_{j\neq i}^Nh_i^\top w_{\mathrm{n},ij}^\mathrm{mV}h_j),
\end{gather}
Their performance is presented in Table~\ref{tab:performance_1}, where it can be observed that they all exhibit performance comparable to that of effective contrastive losses.

% Table generated by Excel2LaTeX from sheet 'Gradient Template'
\begin{table}[ht]\small
  \centering
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}[2]{*}{Type} & \multicolumn{2}{c}{BERT$_\mathrm{base}$} & \multicolumn{2}{c}{RoBERTa$_\mathrm{base}$} \\
          & STS.Avg & TR.Avg & STS.Avg & TR.Avg \\
    \midrule
    Pretrained & 56.70 & 85.34 & 56.57 & 83.20 \\
    \midrule
    $\mathcal{L}_i^\mathrm{info}$ & 76.25 & 85.81 & 76.57 & - \\
    $\mathcal{L}_i^\mathrm{arc}$ & 77.25 & - & 76.60 & - \\
    $\mathcal{L}_i^\mathrm{mpt}$   & 77.25 & 87.56 & 76.42 & 85.10 \\
    $\mathcal{L}_i^\mathrm{met}$   & 78.38 & 87.94 & 77.38 & 85.74 \\
    $\mathcal{L}_i^\mathrm{mat}$   & 77.76 & 88.65 & 76.95 & 85.64 \\
    \midrule
    $\mathcal{L}_i^\mathrm{mMHE}$   & 78.40 & - & 76.91 & - \\
    $\mathcal{L}_i^\mathrm{mMHS}$   & 78.27 & - & 76.37 & - \\
    \midrule
    $\mathcal{L}_i^\mathrm{mB}$    & 78.34 & - & 77.15 & - \\
    $\mathcal{L}_i^\mathrm{mV}$ & 78.24 & - & 76.87 & - \\
    \bottomrule
    \end{tabular}%
  \caption{[TODO]}
  \label{tab:performance_1}%
\end{table}%

==> backup <==
\section{Definitions}

\subsection{Notation}

\begin{itemize}
    \item embeddings
        \begin{align*}
            h_i=(h_{i,1},\cdots,h_{i,D})^\top\in \mathbb{S}^{D-1}
        \end{align*}
    \item views
        \begin{align*}
            h_i, h_i'
        \end{align*}
    \item batch of embeddings
        \begin{align*}
            \{h_i,h_i'\}_{i=1}^N
        \end{align*}
    \item embedding matrix
        \begin{align*}
            H=(h_1,\cdots,h_N)^\top, H'=(h_1',\cdots,h_N')^\top
        \end{align*}
\end{itemize}


\subsection{Desired Gradient}

\begin{align*}
    \frac{\partial \mathcal{L}}{\partial h_i}=\mathrm{GD}(\cdot)\sum_{j=1,j\neq i}^N \mathrm{W}(\cdot)(h_j'-\mathrm{R}(\cdot)h_i')
\end{align*}

\begin{itemize}
    \item Gradient Dissipation
        \begin{align*}
            \mathrm{GD}(i, \{h_k,h_k'\}_{k=1}^N)
        \end{align*}
    \item Weight among samples
        \begin{align*}
            \mathrm{W}(i,j,\{h_k,h_k'\}_{k=1}^N)
        \end{align*}
    \item Ratio between positive and negative samples
        \begin{align*}
            \mathrm{R}(i, j, \{h_k,h_k'\}_{k=1}^N)
        \end{align*}
\end{itemize}

\section{Objectives}

\subsection{Effective Objectives}

\begin{itemize}
    \item InfoNCE
        \begin{align*}
            \mathcal{L}_i=-\log\frac{e^{h_i^\top h_i'/\tau}}{\sum_{j=1}^N e^{h_i^\top h_j'/\tau}}
        \end{align*}
        \begin{align*}
            \frac{\partial \mathcal{L}_i}{\partial h_i}=\frac{1}{\sum_{j=1}^N e^{h_i^\top h_j'/\tau}}\sum_{j=1,j\neq i}^N\frac{e^{h_i^\top h_j'/\tau}}{\tau}(h_j'-h_i')
        \end{align*}
    \item MET
        \begin{align*}
           \mathcal{L}_\mathrm{met}
           =&\max(0, \|h_i-h_i'\|_2\\
           &-\min_{j=1,j\neq i}^N\|h_i-h_j'\|_2+m) 
        \end{align*}\
        \begin{align*}
            \frac{\partial \mathcal{L}_\mathrm{met}}{\partial h_i}
            =&\mathrm{I}_{\{\min_{j=1,j\neq i}^N\|h_i-h_j'\|_2 -\|h_i-h_i'\|_2 < m\}}\\
            &(\frac{1}{\min_{j=1,j\neq i}^N\|h_i-h_j'\|_2}\\
            &(h_j'-\frac{\|h_i-h_j'\|_2}{\|h_i-h_i'\|_2}h_i'))
        \end{align*}
    \item MPT
        \begin{align*}
            \mathcal{L}_\mathrm{mpt}=\max(0,-h_i^\top h_i' + \max_{j=1,j\neq i}^Nh_i^\top h_j'+m)
        \end{align*}
        \begin{align*}
            \frac{\partial \mathcal{L}_\mathrm{mpt}}{\partial h_i}=\mathrm{I}_{\{h_i^\top h_i'-\max_{j=1,j\neq i}^Nh_i^\top h_j'<m\}}(h_j'-h_i')
        \end{align*}
    \item ArcCon
        \begin{align*}
            \theta_{i,j}
            &=\arccos(h_i^\top h_j)\\
            \mathcal{L}_\mathrm{arc}
            &=-\log\frac{e^{\cos(\theta_{i,i'} + m)/\tau}}{e^{\cos(\theta_{i,i'} + m)/\tau}+\sum_{j\neq i}^N e^{h_i^\top h_j'/\tau}}
        \end{align*}
        \begin{align*}
            \frac{\partial \mathcal{L}_\mathrm{arc}}{\partial h_i}
            =&\frac{1}{e^{\cos(\theta_{i,i'} + m)/\tau}+\sum_{j\neq i}^N e^{h_i^\top h_j'/\tau}}\\
            &\sum_{j\neq i}^N\frac{e^{h_i^\top h_j'/\tau}}{\tau}(h_j'-\frac{\sin(\theta_{i,i'}+m)}{\sin(\theta_{i,i'})}h_i')
        \end{align*}
    \item MixCSE
        \begin{align*}
            \tilde{h'}_{i,j}
            =&\frac{\lambda h_i'+(1-\lambda)h_j'}{Z_{i,j}}\\
            Z_{i,j}
            =&\|\lambda h_i'+(1-\lambda)h_j'\|_2\\
            =&\sqrt{1+2\lambda(1-\lambda)h_i'^\top h_j'}\\
            D_i
            =&\sum_{j\neq i}^N(e^{h_i^\top h_j'/\tau}+ e^{h_i^\top \mathrm{SG}(\tilde{h'}_{i,j})/\tau})\\
            \mathcal{L}^\mathrm{mix}_i
            =&
            -\log\frac{e^{h_i^\top h_i'/\tau}}{e^{h_i^\top h_i'/\tau} + D_i}
        \end{align*}
        \begin{align*}
            &\frac{\partial\mathcal{L}_\mathrm{mix}}{\partial h_i}\\
            &=\frac{1}{e^{h_i^\top h_i'/\tau} + D_i}\\
            &\sum_{j\neq i}^N\frac{e^{h_i^\top h_j'/\tau}Z_{i,j} + e^{h_i^\top\tilde{h'}_{i,j}/\tau}(1-\lambda)}{\tau(1-\lambda)}\\
            &(\tilde{h'}_{i,j}-\frac{e^{h_i^\top h_j'/\tau}+e^{h_i^\top\tilde{h'}_{i,j}/\tau}(1-\lambda)}{e^{h_i^\top h_j'/\tau}Z_{i,j}+e^{h_i^\top\tilde{h'}_{i,j}/\tau}(1-\lambda)}h_i')
        \end{align*}
\end{itemize}

\subsection{Ineffective Objectives}

\subsubsection{Alignment \& Uniformity}

\begin{align*}
    \mathcal{L}=\mathcal{L}_\mathrm{a}+ \mathcal{L}_\mathrm{u}
\end{align*}

\begin{itemize}
    \item Alignment
        \begin{align*}
            \mathcal{L}_\mathrm{a}=\frac{1}{N}\sum_{i=1}^N\|h_i-h_i'\|_2^2
        \end{align*}
    \item MHE Uniformity
        \begin{align*}
            \mathcal{L}_\mathrm{u}=\log\frac{1}{N(N-1)}\sum_{i\neq j}^Ne^{-\|h_i-h_j\|_2^2}
        \end{align*}
        \begin{align*}
            \frac{\partial \mathcal{L}_\mathrm{u}}{\partial h_i}
            &=-\frac{2}{N}h_i'+\frac{\sum_{j\neq i}^N2e^{2h_i^\top h_j}h_j}{\sum_{j\neq k}^Ne^{2h_j^\top h_k}}\\
            &=\sum_{j\neq i}^N\frac{2e^{2h_i^\top h_j}}{\sum_{k\neq l}^Ne^{2h_k^\top h_l}}(h_j-\frac{\sum_{k\neq l}^Ne^{2h_k^\top h_l}}{N\sum_{k\neq i}^Ne^{2h_i^\top h_k}}h_i')
        \end{align*}
    \item MHS Uniformity
        \begin{align*}
            \mathcal{L}_{\mathrm{u},i}==-\min_{j\neq i}^N\|h_i-h_j'\|_2
        \end{align*}
        \begin{align*}
            \frac{\partial \mathcal{L}_{\mathrm{u},i}}{\partial h_i}
            &=-\frac{2}{N}h_i'+\frac{1}{\|h_i-h_j'\|_2}h_j'\\
            &=\frac{1}{\|h_i-h_j'\|_2}(h_j'-\frac{2\|h_i-h_j'\|_2}{N}h_i')
        \end{align*}
\end{itemize}

\subsubsection{Non-Contrastive}

\begin{itemize}
    \item BarlowTwins
    \begin{align*}
        W = \frac{1}{N}H^\top H 
    \end{align*}
    \begin{align*}
        \mathcal{L}^\mathrm{BT} 
        =\sum_{i=1}^D(1-W_{i,i})^2+\lambda\sum_{i\neq j}^NW_{i,j}^2
    \end{align*}
    \begin{align*}
        \frac{\partial \mathcal{L}^\mathrm{BT}}{\partial h_i}
        =\frac{2}{N}(&\lambda\sum_{j=1}^N\frac{h_i'^\top h_j'}{N}h_i\\
        &-(I-(1-\lambda)W_\mathrm{diag})h_i'))
    \end{align*}
    \item VICReg
    \begin{align*}
        \mathcal{L}^\mathrm{V}
        &=\sum_{i=1}^N\|h_i-h_i'\|_2^2+\lambda_1\sum_{i=1}^D\max(0, 1-\sqrt{W_{i,i}})\\
        &+\lambda_2\sum_{i\neq j}^DW_{i,j}^2\\
    \end{align*}
    
\end{itemize}

\begin{itemize}
    \item VICReg
        \begin{align*}
            C=HH^\top, NC=\frac{1}{N}H^\top H 
        \end{align*}
        \begin{align*}
            \mathcal{L}_\mathrm{V}
            &=\lambda\sum_{i=1}^N\|h_i-h_i'\|_2^2+\mu\sum_{i=1}^D\max(0, 1-\sqrt{NC_{i,i}})\\
            &+\nu\sum_{i\neq j}^DNC_{i,j}^2\\
            &=\lambda\sum_{i=1}^N\|h_i-h_i'\|_2^2+\mu\sum_{i=1}^D\max(0, 1-\sqrt{NC_{i,i}})\\
            &+\nu(\sum_{i\neq j}^NC_{i,j}^2+\sum_{i}^NC_{i,i}^2-\sum_{i}^DNC_{i,i}^2)\\
            &=\lambda\sum_{i=1}^N\|h_i-h_i'\|_2^2+\mu\sum_{i=1}^D\max(0, 1-\sqrt{NC_{i,i}})\\
            &+\nu(\sum_{i\neq j}^NC_{i,j}^2-\sum_{i}^DNC_{i,i}^2 + N)
        \end{align*}
        \begin{align*}
            \frac{\partial \mathcal{L}_\mathrm{V}}{\partial h_i}
            &=-2\lambda h_i'+\nu\sum_{j\neq i}^N(2h_i^\top h_j)h_j\\
            &=\sum_{j\neq i}^N2\nu h_i^\top h_j(h_j-\frac{\lambda}{\nu\sum_{k\neq i}^Nh_i^\top h_k}h_i')
        \end{align*}
    \item BarlowTwins (BT)
        \begin{align*}
            C=HH'^\top, NC=H^\top H'
        \end{align*}
        \begin{align*}
            \mathcal{L}_\mathrm{BT}
            &=\lambda\sum_{i=1}^D(1-NC_{i,i})^2+\mu\sum_{i\neq j}^NNC_{i,j}^2\\
            &=\lambda\sum_{i=1}^D(1-NC_{i,i})^2\\
            &+\mu(\sum_{i\neq j}^NC_{i,j}^2 + \sum_{i=1}^NC_{i,i}^2-\sum_{i=1}^DNC_{i,i}^2)
        \end{align*}
        \begin{align*}
            \frac{\partial \mathcal{L}_\mathrm{BT}}{\partial h_i}
            &=\mu((2h_i^\top h_i')h_i'+\sum_{j\neq i}^N(2h_i^\top h_j')h_j')\\
            &=\sum_{j\neq i}^N2\mu h_i^\top h_j'(h_j'+\frac{h_i^\top h_i'}{\sum_{k\neq i}h_i^\top h_k'}h_i')
        \end{align*}
\end{itemize}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[ht]\small
  \centering
    \begin{tabular}{c|l|l|l}
    \toprule
    \textbf{Objective} & \multicolumn{1}{c|}{\textbf{Gradient Dissipation}} & \multicolumn{1}{c|}{\textbf{Weight}} & \multicolumn{1}{c}{\textbf{Ratio}} \\
    \midrule
    \midrule
    \multicolumn{4}{c}{\textit{Effective Objectives}} \\
    \midrule
    InfoCSE 
    &       
    $\begin{aligned}
        % \frac{1}{\sum_{j=1}^N e^{h_i^\top h_j'/\tau}}
        1/(\sum_{j=1}^N e^{h_i^\top h_j'/\tau})
    \end{aligned}$
    &       
    $\begin{aligned}
        % \frac{e^{h_i^\top h_j'/\tau}}{\tau}
        (e^{h_i^\top h_j'/\tau})/\tau
    \end{aligned}$
    &  
    \multicolumn{1}{c}{1}
    \\
    MET   
    &       
    $\begin{aligned}
        \mathrm{I}_{\{\min_{j\neq i}^N\|h_i-h_j'\|_2 -\|h_i-h_i'\|_2 < m\}}
    \end{aligned}$
    &       
    $\left\{\begin{aligned}
        &1/\|h_i-h_j'\|_2,\quad\mathrm{else}\\
        &0,\quad j\neq\arg\max_{j\neq i}h_i^\top h_j'
    \end{aligned}\right.$
    &  
    $\begin{aligned}
        \frac{\|h_i-h_j'\|_2}{\|h_i-h_i'\|_2}
    \end{aligned}$
    \\
    MPT   
    &       
    $\begin{aligned}
        \mathrm{I}_{\{h_i^\top h_i'-\max_{j\neq i}^Nh_i^\top h_j'<m\}}
    \end{aligned}$
    &       
    $\begin{aligned}
        \left\{\begin{aligned}
            &1,\quad\mathrm{else}\\
            &0,\quad j\neq\arg\max_{j\neq i}h_i^\top h_j'
        \end{aligned}\right.
    \end{aligned}$
    &  
    \multicolumn{1}{c}{1}
    \\
    ArcCon 
    &       
    $\begin{aligned}
        % \frac{1}{e^{\cos(\theta_{i,i'} + m)/\tau}+\sum_{j\neq i}^N e^{h_i^\top h_j'/\tau}}
        1/(e^{\cos(\theta_{i,i'} + m)/\tau}+\sum_{j\neq i}^N e^{h_i^\top h_j'/\tau})
    \end{aligned}$
    &       
    $\begin{aligned}
        % \frac{e^{h_i^\top h_j'/\tau}}{\tau}
        e^{h_i^\top h_j'/\tau}/\tau
    \end{aligned}$
    &  
    $\begin{aligned}
        \frac{\sin(\theta_{i,i'}+m)}{\sin(\theta_{i,i'})}
    \end{aligned}$
    \\
    MixCSE 
    &       
    $
        % \frac{1}{e^{h_i^\top h_i'/\tau}+\sum_{j\neq i}^N(e^{h_i^\top h_j'/\tau}+e^{h_i^\top \tilde{h'}_{i,j}/\tau})}
        % 1/(e^{h_i^\top h_i'/\tau}+\sum_{j\neq i}^N(e^{h_i^\top h_j'/\tau}+e^{h_i^\top \tilde{h'}_{i,j}/\tau}))
        1/(D_i+\sum_{j\neq i}e^{h_i^\top \tilde{h'}_{i,j}/\tau})
    $
    &       
    $
        % \frac{e^{h_i^\top h_j'/\tau}+e^{h_i^\top\tilde{h'}_{i,j}/\tau}\frac{(1-\lambda)}{Z_{i,j}}}{\tau}
        (e^{h_i^\top h_j'/\tau}+e^{h_i^\top\tilde{h'}_{i,j}/\tau}\frac{(1-\lambda)}{Z_{i,j}})/\tau
    $
    &  
    $
        \frac{1 + e^{h_i^\top(\tilde{h'}_{i,j}-h_j')/\tau}(1-\frac{\lambda}{Z_{i,j}})}{1 + e^{h_i^\top(\tilde{h'}_{i,j}-h_j')/\tau}(\frac{1-\lambda}{Z_{i,j}})}
    $
    \\
    \midrule
    \midrule
    \multicolumn{4}{c}{\textit{Ineffective Objectives}} \\
    \midrule
    MHE   
    &       
    \multicolumn{1}{c|}{1}
    &       
    $\begin{aligned}
        \frac{2e^{2h_i^\top h_j}}{\sum_{k\neq l}^Ne^{2h_k^\top h_l}}
    \end{aligned}$
    &  
    $\begin{aligned}
        \frac{\sum_{k\neq l}^Ne^{2h_k^\top h_l}}{N\sum_{k\neq i}^Ne^{2h_i^\top h_k}}
    \end{aligned}$
    \\
    MHS   
    &       
    \multicolumn{1}{c|}{1}
    &       
    $\left\{\begin{aligned}
        &\frac{1}{\|h_i-h_j'\|_2},\quad\mathrm{else}\\
        &0,\quad j\neq\arg\max_{j=1,j\neq i}h_i^\top h_j'
    \end{aligned}\right.$
    &  
    $\begin{aligned}
        \frac{2\|h_i-h_j'\|_2}{N}
    \end{aligned}$
    \\
    VICReg 
    &       
    \multicolumn{1}{c|}{1}
    &       
    $\begin{aligned}
        2\nu h_i^\top h_j
    \end{aligned}$
    &  
    $\begin{aligned}
        \frac{\lambda}{\nu\sum_{k\neq i}^Nh_i^\top h_k}
    \end{aligned}$
    \\
    BT 
    &       
    \multicolumn{1}{c|}{1}
    &       
    $\begin{aligned}
        2\mu h_i^\top h_j'
    \end{aligned}$
    &  
    $\begin{aligned}
        -\frac{h_i^\top h_i'}{\sum_{k\neq i}h_i^\top h_k'}
    \end{aligned}$
    \\
    \midrule
    \midrule
    \multicolumn{4}{c}{\textit{Our Modifications}} \\
    \midrule
    M-MHE
    &
    $\begin{aligned}
        \mathrm{I}_{\{h_i^\top h_i'-\max_{j\neq i}^Nh_i^\top h_j'<m\}}
    \end{aligned}$
    &
    $\begin{aligned}
        \frac{e^{h_i^\top h_j}/\tau}{\tau\sum_{k\neq l}^Ne^{h_k^\top h_l/\tau}}
    \end{aligned}$
    &
    \multicolumn{1}{c}{1}
    \\
    M-MHS
    &
    $\begin{aligned}
        \mathrm{I}_{\{h_i^\top h_i'-\max_{j\neq i}^Nh_i^\top h_j'<m\}}
    \end{aligned}$
    &
    $\left\{\begin{aligned}
        &\frac{1}{\|h_i-h_j'\|_2},\quad\mathrm{else}\\
        &0,\quad j\neq\arg\max_{j=1,j\neq i}h_i^\top h_j'
    \end{aligned}\right.$
    &
    \multicolumn{1}{c}{1.25}
    \\
    M-VICReg
    &
    $\begin{aligned}
        \mathrm{I}_{\{h_i^\top h_i'-\max_{j\neq i}^Nh_i^\top h_j'<m\}}
    \end{aligned}$
    &
    $\begin{aligned}
        \frac{e^{h_i^\top h_j}/\tau}{\tau\sum_{k\neq l}^Ne^{h_k^\top h_l/\tau}}
    \end{aligned}$
    &
    \multicolumn{1}{c}{1.75}
    \\
    M-BT
    &
    $\begin{aligned}
        \mathrm{I}_{\{h_i^\top h_i'-\max_{j\neq i}^Nh_i^\top h_j'<m\}}
    \end{aligned}$
    &
    $\begin{aligned}
        \frac{e^{h_i^\top h_j'}/\tau}{\tau\sum_{k\neq l}^Ne^{h_k^\top h_l'/\tau}}
    \end{aligned}$
    &
    \multicolumn{1}{c}{1.25}
    \\
    \bottomrule
    \end{tabular}%
  \caption{TODO}
  \label{tab:gd_w_r}%
\end{table*}%

% \begin{itemize}
%     \item MixCSE
%     \begin{itemize}
%         \item GD
%             \begin{align*}
%                 \frac{1}{e^{h_i^\top h_i'/\tau}+\sum_{j\neq i}^N(e^{h_i^\top h_j'/\tau}+e^{h_i^\top \tilde{h'}_{i,j}/\tau})}
%             \end{align*}
%         \item W
%             \begin{align*}
%                 &\frac{e^{h_i^\top h_j'/\tau}Z_{i,j}+e^{h_i^\top\tilde{h'}_{i,j}/\tau}(1-\lambda)}{Z_{i,j}\tau}\\
%                 =&e^{h_i^\top h_j'/\tau}\frac{1}{\tau}+e^{h_i^\top\tilde{h'}_{i,j}/\tau}\frac{(1-\lambda)}{\tau Z_{i,j}}\\
%                 =&\frac{e^{h_i^\top h_j'/\tau}+e^{h_i^\top\tilde{h'}_{i,j}/\tau}\frac{(1-\lambda)}{Z_{i,j}}}{\tau}
%             \end{align*}
%         \item R
%             \begin{align*}
%                 &\frac{e^{h_i^\top h_j'/\tau}Z_{i,j}+e^{h_i^\top\tilde{h'}_{i,j}/\tau}(Z_{i,j}-\lambda)}{e^{h_i^\top h_j'/\tau}Z_{i,j}+e^{h_i^\top\tilde{h'}_{i,j}/\tau}(1-\lambda)}\\
%                 =&\frac{1 + \frac{e^{h_i^\top\tilde{h'}_{i,j}/\tau}}{{e^{h_i^\top h_j'/\tau}}}(1-\frac{\lambda}{Z_{i,j}})}{1 + \frac{e^{h_i^\top\tilde{h'}_{i,j}/\tau}}{{e^{h_i^\top h_j'/\tau}}}(\frac{1-\lambda}{Z_{i,j}})}\\
%                 =&\frac{1 + e^{h_i^\top(\tilde{h'}_{i,j}-h_j')/\tau}(1-\frac{\lambda}{Z_{i,j}})}{1 + e^{h_i^\top(\tilde{h'}_{i,j}-h_j')/\tau}(\frac{1-\lambda}{Z_{i,j}})}
%             \end{align*}
%     \end{itemize}
% \end{itemize}



\section{Introduction}

These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

% Entries for the entire Anthology, followed by custom entries
\bibliography{anthology,custom,ACL24}
\bibliographystyle{acl_natbib}
